Learn2Chat: Rethinking Dyadic Talking Heads via Interaction-Modulated Monologic Priors

Dyadic conversational motion generation is essential for realistic interactive digital humans. Existing approaches typically model conversational behaviors within unified dyadic generators. However, such holistic formulations tend to couple self-speech-driven motion with partner-responsive social feedback, leaving the interaction-specific component implicit and underutilizing the speech-motion correspondence already learned by pretrained monologic motion models. We propose Learn2Chat, a unified framework that models dyadic motion as interaction modulation over pretrained monologic motion priors. This design separates intrinsic speech-driven motion from social interaction effects and enables more structured interaction modeling. Specifically, we introduce a Monologic-Anchored Motion Factorization scheme that leverages the semantic motion manifold learned from monologic data to disentangle audio-driven motion dynamics from interaction-induced modulation, yielding clean interaction representations from dyadic sequences. On top of this representation space, a Cross-Attentive Interaction Latent Prediction module maps paired speech signals to interaction latents through cross-branch attention and interaction alignment. During inference, the predicted interaction latents modulate canonical monologic motion to generate coherent and synchronized dyadic behaviors in a data-efficient manner. Extensive experiments on the DualTalk benchmark demonstrate that Learn2Chat achieves state-of-the-art performance across both quantitative metrics and perceptual evaluations. Moreover, the framework is model-agnostic and seamlessly integrates with diverse pretrained monologic motion backbones, highlighting the effectiveness of prior reuse and interaction adaptation for scalable conversational motion generation. More visual results are available on the project page.

==> rebuttal/sec/intro.tex <==
\noindent We thank the reviewers for their constructive comments and address their main concerns below.

==> rebuttal/sec/r1.tex <==
\rone{R\#crmm-W1: Overview fig.} We agree that Fig. 2 is visually dense and will simplify the overview and split the detailed pipeline into clearer subfigures in the revision.

\rone{R\#crmm-W2/W3 \& R\#crmm-S3: Limitation discussion.}
% As noted in Sec.5, our current method generates dyadic interaction motion from audio signals alone and does not model visual feedback, such as eye-gaze dynamics. We emphasize that this limitation primarily arises from the scarcity of high-quality, fine-grained conversational motion datasets, rather than from an intrinsic constraint of our framework. Accurate modeling of gaze interactions requires precise estimation of eyeball movements, which existing 3D head reconstruction methods predominantly capture only at the global head level. In addition, predicting gaze behavior depends on knowledge of interlocutors' relative orientations, information typically absent in available datasets. Consequently, simultaneous modeling of head and eye movements remains challenging.
% While we cannot include videos or external links due to rebuttal constraint, we acknowledge the importance of studying failure cases and plan to provide a more detailed discussion and illustrative examples in the final version of the paper.
We agree that audio-only cues cannot fully capture the closed-loop nature of face-to-face interaction. Visual feedback, such as gaze and partner motion, could further improve fine-grained listener reactions, including gaze shifts, mutual attention, and visually grounded nods.
% Our current setting follows the audio-only DualTalk protocol, and we will include visual examples and a clearer discussion of these missing cues in the revision.
Our setting focuses on generating the motions of both participants solely from duet audio, without relying on GT visual observations of the partner. While gaze feedback could further enrich interaction behaviors, incorporating such cues remains challenging due to the lack of large-scale datasets with reliable gaze annotations and consistent spatial information. We will expand this discussion in the revision.

\rone{R\#crmm-S1/S2: Video comparisons.}
Due to rebuttal policy, we cannot add new videos or external links at this stage. We will include side-by-side comparisons with ground-truth motion and NN baselines in our revised video demo.

\rone{R\#crmm-S4: Clarification on metrics.}
% SID~[23] quantifies the diversity of predicted motions by clustering sequences with k-means and computing the average Shannon entropy.
% Higher SID indicates more varied outputs， while FD/P-FD measure fidelity to the ground-truth motions.
% These metrics are complementary: SID captures motion diversity, FD/P-FD capture fidelity, and a comprehensive evaluation should consider both aspects.
% SID measures diversity, FD/P-FD measure fidelity, and both are needed for a complete evaluation.
SID~[23] measures motion diversity by clustering generated sequences with k-means and computing the average Shannon entropy. In contrast, FD/P-FD measure fidelity to ground-truth motions. Both metrics are complementary and needed for a comprehensive evaluation.

\rone{R\#crmm-S5-6: Experimental setting clarification.}
Yes, our method assumes two separated audio streams, following the standard setting of prior dyadic motion generation works~[23,27,37]. For single-channel recordings, speaker separation can be applied first; in fact, DualTalk obtains its separated audio tracks in this way.
For dyadic baselines, their original setting uses ground-truth partner motion as input, which is not available in our audio-only setting and would give them an unfair advantage. Therefore, we replace the ground-truth partner motion with monologic motions generated by the same pretrained backbones~[16,9] used in our method, and fine-tune all baselines under this setting. This ensures all methods use the same input information.

\rone{R\#crmm-S7 \& R\#9cxi-W2: Perceptual evaluation.}
We have included a user study in Sec.2.1 of the supplementary material, where participants compare different methods in terms of interaction naturalness, lip synchronization, and overall motion quality. Our method is consistently preferred over all baselines, supporting that the generated behaviors are perceptually meaningful rather than only numerically better. 

==> rebuttal/sec/r2.tex <==

\rtwo{R\#9cxi-W1: Lip synchronization evaluation.}
% Our method employs the FLAME parametric motion model, where lip articulation is predominantly driven by the predicted jaw parameters. The jaw-related metrics reported in Tables 1-2 already capture the accuracy of lip movements. To provide a more direct and widely recognized assessment, we additionally computed the Lip Vertex Error~(LVE), a standard metric in audio-driven talking head research. The results shown above confirm that our method maintains accurate lip synchronization while simultaneously modeling dyadic interaction dynamics, indicating that speaking quality is preserved alongside reactive listening behaviors.
Our method adopts the FLAME parametric motion model, where lip articulation is mainly controlled by the predicted jaw params. The jaw-related metrics in Tab.~1--2 already reflect lip motion accuracy.
To further provide an explicit evaluation, we additionally compute Lip Vertex Error (LVE), a widely used lip synchronization metric in talking-head generation. As shown in the Tab.~\ref{lve}, our method achieves the lowest LVE under both Test and OOD settings, demonstrating that modeling dyadic interaction does not degrade speaking quality while preserving accurate lip synchronization.
\input{tab/lve}


% \vspace{-0.5mm}
\rtwo{R\#9cxi-W3: Granularity of interactive behaviors.}
To analyze listening behaviors, we exploit the separated audio tracks to determine speaker/listener roles and report role-specific metrics. As shown in the upper part of Tab.~\ref{listener}, our method consistently improves performance for the listener role compared with monologic baselines.
These improvements indicate that the model learns responsive listening dynamics rather than simply reproducing speaking motions or remaining static during listening segments. The gains in both motion fidelity and diversity metrics suggest that listener motions vary according to conversational context. We will provide a detailed discussion of role-specific behaviors in the revision.
\input{tab/listener_diffmono} 

\noindent\uline{Note to \rtwo{R\#9cxi:} We hope the added evidence clarifies that our model does learn to ``listen'', rather than simply producing muted or static listener motions, and we respectfully ask the reviewer to re-evaluate our work.}

==> rebuttal/sec/r3.tex <==
\rthree{R\#C6y4-W1: Generalization across monologic predictors.}
To test plug-and-play generalization, in the lower part of Tab.~\ref{listener}, we train Learn2Chat with one monologic predictor and replace it with another at inference, e.g., Ours([16]@[9]) means training with [16] and inference with [9]. The results remain stable, indicating that the learned interaction modulation is not tied to a single monologic backbone.

\rthree{R\#C6y4-W2 \& R\#C6y4-S1: Architecture design and novelty.}
% We would like to clarify the design of our framework. The Semantics Encoder $E_S$ and Semantics-Interaction Decoder $D$ are shared for both monologic and dyadic motion generation, while the Interaction Encoder $E_I$is only applied to dyadic motion. This sharing strategy ensures that the overall architectural complexity remains within a reasonable range. Compared to other dyadic interaction methods, the additional trainable parameters introduced by our framework strike a favorable balance between model complexity and performance~(Tab.3).
% While the use of swap and cycle consistency losses for disentanglement is not entirely novel in other domains, our work is the first to adopt this factorization strategy to explicitly formulate dyadic interaction learning. The reformulation itself is non-trivial and is central to our contribution. In particular, the novel generation diagram illustrating interaction-modulated monologic priors is the core innovation of our work, rather than the specific choice of loss functions. This design enables effective separation of speech-driven semantics from interaction-induced modulation, which is critical for generating realistic dyadic behaviors.
The Semantics Encoder and Semantics-Interaction Decoder are shared for monologic and dyadic motion, while only the Interaction Encoder is added for dyadic modeling. Thus, the extra design is focused on interaction factorization rather than introducing a large standalone dyadic generator.  
As shown in Tab.~3, the additional parameters remain small compared with existing dyadic frameworks.
While swap and cycle losses are common tools, our novelty lies in using monologic priors to formulate dyadic generation as interaction modulation, separating speech-driven motion from partner-conditioned interaction.


==> rebuttal/tab/listener_diffmono.tex <==
\begin{table}[h]
    \vspace{-5mm}
    \caption{Listener and plug-and-play results.}
    \resizebox{1.0\linewidth}{!}{
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{@{}c|ccc|ccc|ccc|ccc|ccc@{}}
    \bottomrule
    \multirow{3}{*}{\textbf{Methods}}  & \multicolumn{3}{c|}{\textbf{FD $\downarrow$}}                                                                                                          & \multicolumn{3}{c|}{\textbf{P-FD $\downarrow$}}                                                                                                        & \multicolumn{3}{c|}{\textbf{MSE $\downarrow$}}                                                                                                                                                       & \multicolumn{3}{c|}{\textbf{SID $\uparrow$}}    & \multicolumn{3}{c}{\textbf{rPCC $\downarrow$}}                                                                                                                                                       \\ \cline{2-16}
                                        & exp               & \begin{tabular}[c]{@{}c@{}}jaw\\ $\times 10^{-3}$ \end{tabular} & \begin{tabular}[c]{@{}c@{}}pose\\ $\times 10^{-2}$ \end{tabular} & exp               & \begin{tabular}[c]{@{}c@{}}jaw\\ $\times 10^{-3}$ \end{tabular} & \begin{tabular}[c]{@{}c@{}}pose\\ $\times 10^{-2}$ \end{tabular} & \begin{tabular}[c]{@{}c@{}}exp\\ $\times 10^{-1}$ \end{tabular} & \begin{tabular}[c]{@{}c@{}}jaw\\ $\times 10^{-3}$ \end{tabular} & \begin{tabular}[c]{@{}c@{}}pose\\ $\times 10^{-2}$ \end{tabular} & exp              & jaw              & pose      & \begin{tabular}[c]{@{}c@{}}exp\\ $\times 10^{-2}$ \end{tabular} & \begin{tabular}[c]{@{}c@{}}jaw\\ $\times 10^{-1}$ \end{tabular} & \begin{tabular}[c]{@{}c@{}}pose\\ $\times 10^{-1}$ \end{tabular} \\ \hline
    \multicolumn{16}{c}{\textbf{Listener}~(Test/OOD)} \\ \hline
    {[}16{]}                            & 30.98/31.54       & 5.31/5.26                                                       & 3.00/2.85                                                        & 31.02/31.82       & 5.31/5.27                                                       & 3.24/3.07                                                        & 6.72/6.81                                                       & 1.76/1.75                                                       & 2.05/2.04                                                        & 1.42/1.46        & 1.44/1.32        & 1.67/1.68 & 15.88/15.35                                                     & 2.48/2.16                                                       & 2.09/1.85                                                        \\
    {[}9{]}                             & 30.79/31.08       & 5.30/5.28                                                       & 2.91/2.79                                                        & 30.79/31.07       & 5.30/5.26                                                       & 3.14/3.01                                                        & 6.74/6.82                                                       & 1.77/1.75                                                       & 1.85/1.86                                                        & 1.43/1.51        & 1.39/1.38        & 1.72/1.74 & 15.75/15.18                                                     & 2.49/2.12                                                       & 2.58/2.12                                                        \\ \hline
    Ours({[}16{]})                      & 15.50/22.85       & 1.80/2.62                                                       & 2.13/2.01                                                        & 16.61/23.98       & 1.91/2.72                                                       & 2.36/2.23                                                        & 4.53/6.14                                                       & 1.11/1.41                                                       & 1.57/1.59                                                        & 3.02/2.70        & 2.22/2.04        & 1.87/1.85 & 6.89/7.70                                                       & 1.38/1.49                                                       & 1.62/1.41                                                        \\
    Ours({[}9{]})                       & 15.08/22.97       & 1.80/2.67                                                       & 2.43/2.34                                                        & 16.23/24.14       & 1.91/2.78                                                       & 2.67/2.56                                                        & 4.55/6.29                                                       & 1.12/1.44                                                       & 1.71/1.73                                                        & 3.05/2.73        & 2.23/2.01        & 1.75/1.70 & 6.62/7.46                                                       & 1.39/1.51                                                       & 1.57/1.38                                                        \\ \hline
    \multicolumn{16}{c}{\textbf{Plug-and-Play with Different Monologic Baselines}~(Trained@Inference, Test/OOD)} \\ \hline
    Ours({[}16{]}@{[}9{]})              & 15.05/22.66       & 2.23/3.03                                                       & 6.01/6.12                                                        & 16.09/23.76       & 2.33/3.13                                                       & 5.98/6.44                                                        & 4.63/6.32                                                       & 1.31/1.60                                                       & 2.34/2.64                                                        & 3.07/2.75        & 2.09/1.92        & 1.80/1.75 & 6.87/7.63                                                       & 1.46/1.52                                                       & 2.70/2.52                                                        \\
    Ours({[}9{]}@{[}16{]})              & 15.78/23.00       & 1.86/2.54                                                       & 5.46/5.65                                                        & 16.80/24.07       & 1.96/2.64                                                       & 5.82/5.82                                                        & 4.68/6.27                                                       & 1.18/1.42                                                       & 2.27/2.53                                                        & 3.07/2.76        & 2.24/2.05        & 1.39/1.36 & 6.96/7.91                                                       & 1.39/1.50                                                       & 2.59/2.49                                                        \\
    \toprule
    \end{tabular}}
    \vspace{-2mm}
    \label{listener}
\end{table} 

==> rebuttal/tab/lve.tex <==
% \begin{table}[]
%     \begin{tabular}{c|c}
%     \hline
%     \textbf{Methods}                 & \begin{tabular}[c]{@{}c@{}}\textbf{LVE}\\ Test/OOD\end{tabular} \\ \hline
%     {[}23{]}({[}16{]})               & 13.95/13.48                                                     \\
%     {[}23{]}({[}9{]})                & 14.01/13.51                                                     \\
%     {[}37{]}({[}16{]})               & 11.15/11.32                                                     \\
%     {[}37{]}({[}9{]})                & 11.00/11.05                                                     \\
%     {[}27{]}({[}16{]})               & 9.88/10.59                                                      \\
%     {[}27{]}({[}9{]})                & 9.85/10.60                                                      \\ \hline
%     \rowcolor{gray!20}Ours({[}16{]}) & \underline{9.16}/\underline{9.98}                               \\
%     \rowcolor{gray!20}Ours({[}9{]})  & \textbf{9.15}/\textbf{9.83}                                     \\ \hline
%     \end{tabular}
% \end{table}
% \begin{table}[]
%     \resizebox{1.1\linewidth}{!}{
%     \begin{tabular}{c|cc|cccccc}
%     \hline
%     \textbf{Methods}        & \textbf{Ours([16])}               & \textbf{Ours([9])}          & {[}23{]}([16]) & {[}23{]}([9]) & {[}37{]}([16]) & {[}37{]}([9]) & {[}27{]}([16]) & {[}27{]}([9]) \\ \hline
%     \textbf{LVE (Test/OOD)} & \underline{9.16}/\underline{9.98} & \textbf{9.15}/\textbf{9.83} & 13.95/13.48    & 14.01/13.51   & 11.15/11.32    & 11.00/11.05   & 9.88/10.59     & 9.85/10.60 \\ \hline
%     \end{tabular}}
% \end{table}
\begin{table}[h]
    \centering
    \vspace{-5mm}
    \caption{LVE comparison.}
    \resizebox{1.0\linewidth}{!}{
    \renewcommand{\arraystretch}{1.5}
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c|cc|cccccc}
    \hline
    \textbf{Methods}        & \cellcolor{gray!20}\textbf{Ours([16])}               & \cellcolor{gray!20}\textbf{Ours([9])}          & {[}23{]}([16]) & {[}23{]}([9]) & {[}37{]}([16]) & {[}37{]}([9]) & {[}27{]}([16]) & {[}27{]}([9]) \\ \hline
    \textbf{LVE (Test/OOD)} & \cellcolor{gray!20}\underline{9.16}/\underline{9.98} & \cellcolor{gray!20}\textbf{9.15}/\textbf{9.83} & 13.95/13.48    & 14.01/13.51   & 11.15/11.32    & 11.00/11.05   & 9.88/10.59     & 9.85/10.60    \\ \hline
    \end{tabular}}
    \vspace{-2mm}
    \label{lve}
\end{table} 
